Lang--Trotter Conjecture for CM Elliptic Curves

Given an elliptic curve $E$ over $\mathbb{Q}$ and non-zero integer $r$, the Lang--Trotter conjecture predicts a striking asymptotic formula for the number of good primes $p\leqslant x$, denoted by $\pi_{E,r}(x)$, such that the Frobenius trace of $E$ at $p$ is equal to the given integer $r$. We focus on the CM case in this memoir, and show how to realize the following two goals: (1) to give an unconditional estimate for $\pi_{E,r}(x)$, which confirms the upper bound part of the conjecture up to a constant multiple; (2) to give a conditional explicit asymptotic formula for $\pi_{E,r}(x)$ based on the Hardy--Littlewood conjecture on primes represented by quadratic polynomials. For completeness, we also summarize classical results on quadratic, cubic and quartic residues, as well as the corresponding reciprocity laws. This part should be of independent interests and could provide useful materials for more junior readers. We also highlight some possible extensions of the arguments in this memoir that may work for other statistical problems of CM elliptic curves.

==> notationindex.tex <==
\chapter*{Notation index}

We list some of the notation used in this book that may not be
standard. Further notation and conventions are explained in
Section~\ref{21}. Some notation that is local to a single chapter are
omitted.

\newcommand{\pg}[1]{p. \pageref{#1}}
\newcommand{\pgb}[1]{\pageref{#1}}
\par
\bigskip
\par

{\small
  \begin{longtable}{lll}
    $\mathcal{F}_N$ & family of modular form &
                                               \pg{sec-general}
    \\
    $M(f)$ & mollifier & \pg{pg-mollifier}
 \\
    $C_f(t)$ & correlation of~$t$ with modular symbols & \pg{pg-cft}
  \end{longtable}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "moment-theory"
%%% TeX-PDF-mode: t
%%% End: 

